VARGAN: Variance Enforcing Network Enhanced GAN

Generative adversarial networks (GANs) are one of the most widely used generative models. GANs can learn complex multi-modal distributions, and generate real-like samples. Despite the major success of GANs in generating synthetic data, they might suffer from unstable training process, and mode collapse. In this paper, we introduce a new GAN architecture called variance enforcing GAN (VARGAN), which incorporates a third network to introduce diversity in the generated samples. The third network measures the diversity of the generated samples, which is used to penalize the generator's loss for low diversity samples. The network is trained on the available training data and undesired distributions with limited modality. On a set of synthetic and real-world image data, VARGAN generates a more diverse set of samples compared to the recent state-of-the-art models. High diversity and low computational complexity, as well as fast convergence, make VARGAN a promising model to alleviate mode collapse.

==> Tables/Accuracy_EES.tex <==
\noindent\adjustbox{max width=\textwidth}{
\begin{tabular}{llcrrll}
\toprule
                    GAN architecture              & Design & Category & \multicolumn{3}{c}{Partial Image}\\ 
                    % & & \multicolumn{3}{l}{Full Image} \\ 
                                  \cline{4-6}  
                                   & & &HP     & LP \\ \hline
                                  

% - &GAN& $9\times9$ & & 4,230 &3,025 & &2,650 & 1,417\\
\midrule
cGAN& $9\times9$ & - & 98 & 95\\
cGAN& $9\times9$ & DSGAN & 98 & 95 \\
cGAN& $9\times9$ &  MB Discr&98 & 95 \\
cGAN& $9\times9$ &  PacGAN& 84 & 67\\

\midrule

cCGAN& $9\times9$ & - & 77 & 49\\
cCGAN& $9\times9$ & DSGAN & 85 & 61\\
cCGAN& $9\times9$ & MB Discr & \\ 
cCGAN& $9\times9$ & PacGAN & 73 & 47\\
\midrule
GAN& $9\times9$ & - & 70 & 30 \\
GAN& $9\times9$ & DSGAN & 71 & 28 \\ 
GAN& $9\times9$ & MB Discr & 70 & 30 \\
GAN& $9\times9$ &  PacGAN & 71 & 29\\
\midrule
CGAN& $9\times9$ & - & 36 & 17 \\
CGAN& $9\times9$ & DSGAN& 39 & 17\\ 
CGAN& $9\times9$ & MB Discr& 37 & 17\\
CGAN& $9\times9$ &  PacGAN& 48 & 21\\

\midrule
\midrule

cGAN& $19\times19$ & - & 77 & 24\\
cGAN& $19\times19$  & DSGAN & 72 & 30 \\
cGAN& $19\times19$ &  MB Discr & 72 & 28\\
cGAN& $19\times19$  & PacGAN & 44 & 54 \\
\midrule
cCGAN& $19\times19$  & - &41 & 50\\
cCGAN& $19\times19$  & DSGAN & 54 & 41\\
cCGAN& $19\times19$  & MB Discr & 20 & 74 \\
cCGAN& $19\times19$  & PacGAN & 14 & 60\\
\midrule
GAN& $19\times19$  & - & 74 & 25\\
GAN& $19\times19$  & DSGAN & 65 & 34\\
GAN& $19\times19$  & MB Discr & 62 & 37 \\
GAN& $19\times19$  & PacGAN & 74 & 25\\
\midrule
CGAN& $19\times19$  & - & 38 & 61\\
CGAN& $19\times19$  & DSGAN & 36 & 63\\
CGAN& $19\times19$  & MB Discr &  24 & 75\\
CGAN& $19\times19$  & PacGAN & 32 & 67\\
\bottomrule
\end{tabular}}


==> Tables/CGAN-comparison-categories.tex <==

% \begin{tabular}{|c|c|c|c|p{0.5cm}|c|c|c|c|p{0.5cm}|p{0.6cm}|p{0.6cm}|c|c|}
\noindent\adjustbox{max width=\textwidth}{

\begin{tabular}{ccccccccccccc}
\toprule
 \multirow{6}{*}{Model} &  \multirow{6}{*}{Design} &  
 \multirow{6}{*}{Category} &
 \multicolumn{9}{c}{Category Names}\\
 \cline{4-13}
 & & & \multicolumn{5}{c}{HP} & SUM &\multicolumn{3}{c}{LP}& SUM\\
 \cline{4-8}
 \cline{10-12}
 &  &  & DC Block  & DC Block  & DC Block  & DC Block & DC Block&  & DC Pass  & DC Pass & DC Pass\\
 & & & Band Pass & Band Pass Stop & High Pass & True High Pass &  Very High Pass & &Band Stop & Low Pass & Stop Pass\\
\toprule
\multirow{2}{*}{cGAN}&  \multirow{2}{*}{$9\times9$} & Total in data & 2,804 & 2,614 & 3,206 & 8,556 & 5,537 &22,717& 4,193 & 4,467 & 1,391 & 10,051\\
& & 8 Categories & 1,272 & 1,383 & 1,819 & 5,819 & 2,934 &13,227& 2,851 & 2,400 & 750& 6,001\\
& & \% & 45 & 53 & 57 & 68 & 53 & 58 & 68 & 54 & 54 & 59\\
\midrule
\multirow{2}{*}{cGAN}&  \multirow{2}{*}{$9\times9$} & Total in data & 2,804 & 2,614 & 3,206 & -&- &8,624& 4,193 & 4,467 & 1,391 & 10,051\\
& & 6 Categories & 1,081 & 1,613 & 1,783 & -& - &4,477& 2,866 & 1,985 & 662 &5,513\\
& & \% & 39 & 61 & 56& - & - &51& 68& 44& 47& 54\\
\midrule
\multirow{2}{*}{cGAN}&  \multirow{2}{*}{$9\times9$} & Total in data &-&-& -&-&-& 22,717&-&-&-&10,051\\
& & 2 Categories  &-&-& - &-&-& 11,402&-&-&-& 6,251\\
& & \%  &-&-& -&-&-& 50&-&-&-&62\\

\midrule
\midrule
\multirow{2}{*}{cCGAN}& 
\multirow{2}{*}{$9\times9$} & Total in data & 2,804 & 2,614 & 3,206 & 8,556 & 5,537 &22,717& 4,193 & 4,467 & 1,391 & 10,051\\
& & 8 Categories & 2,275 & 2,204& 2,653 & 7,061 & 4,574 &18,867& 3,538 & 3,765 & 1,175& 8,478 \\
& & \% & 81 & 84 & 83 & 82 & 83 &83 & 84 & 84 & 84& 84 \\
\midrule
\multirow{2}{*}{cCGAN}&  \multirow{2}{*}{$9\times9$} & Total in data & 2,804 & 2,614 & 3,206 & -&- &8,624& 4,193 & 4,467 & 1,391 & 10,051\\
& & 6 Categories & 1,901 & 2,027 & 2,596 & -&- && 3,736 & 3,593 & 1,197  \\
& & \% & 67 & 77 & 81 & - & - && 89 & 80 & 86 \\

\midrule
\multirow{2}{*}{cCGAN}&  \multirow{2}{*}{$9\times9$} & Total in data  &-&-& - &-&-&22,717 &-&-&-&10,051\\
& & 2 Categories  &-&-& - &-&-&9,306 &-&-&-&4,624\\
& & \%  &-&-& - &-&-& 40&-&-&-&46\\
\bottomrule
% etc. ...
\end{tabular}}

==> Tables/Complexity_time_comparison.tex <==
\begin{tabular}{lllllllll}

Dataset & GAN & GAN + MB & DSGAN & PacGAN & MADGAN & GDPP & VARGAN & PacVARGAN \\ \midrule
Ring 8 modes&    &  693.2 $\pm$ 26.3&  &  & 1,393.3  $\pm$ 73.3  & 1,962.4 $\pm$ 182.39 & 1,480.4 $\pm$  31.1 &
1,477.0 $\pm$  16.1 \\ 
Grid 25 modes &  & 962.4 $\pm$ 2.653 &  &  &   1,679.0 $\pm$ 81.0 & 2,463.0 $\pm$ 85.2 & 814.6 $\pm$  23.6 &
833.2 $\pm$ 3.6\\
Grid 36 modes    &  & 1,136.4 $\pm$ 4.1 &  &  & 1,804.0 $\pm$ 3.93& 2,712.6 $\pm$ 306.9 && \\




\midrule
\midrule
Stacked MNIST FF &  &  &  &  & 973.9 $\pm$ 12.2& 2,312.7 $\pm$ 35.4 &&  \\
Stacked MNIST Conv &  &  &  &  & 1,102.8 $\pm$ 10.9 & 379.5 $\pm$ 1.1&  \\
\midrule
\midrule

EES $9\times9$ FF &  677.6 $\pm$ 9.3 & 672.8 $\pm$ 12.0 & 838.0 $\pm$ 12.3 & 663.4 $\pm$ 1.8 &  & 2,969.4 $\pm$ 19.5 & 996.2 $\pm$ 13.0 & 929.2 $\pm$ 4.1\\ 
EES  $9\times9$ Conv & 3,704.2 $\pm$   1,083.7 &  18,133.6 $\pm$   1,805.4&  1,844.5 $\pm$   6.8&    1,384.6  $\pm$  32.5&  & 3,036.2 $\pm$ 66.8 & 1,841.2 $\pm$ 487.96 & 3072.6 $\pm$ 1130.2  \\
\midrule
EES  $19\times19$ FF &  439.6 $\pm$ 12.1 & 448.7 $\pm$ 29.0 &  440.2 $\pm$ 14.5 &  369.2 $\pm$ 30.1&  & 1241.6 $\pm$ 38.03 &  673.2 $\pm$ 52.1 &  637.4 $\pm$ 21.7\\
EES $19\times19$ Conv & 975.4 $\pm$  60.9 & 3,766.8 $\pm$  60.0  &   1,447.6 $\pm$  10.5 & 908.8 $\pm$ 11.4 &  & 1,562.6 $\pm$ 73.9 & 1,219.8 $\pm$ 45.7 & 1,126.4 $\pm$ 12.5 \\
 \bottomrule
\end{tabular}


==> Tables/EES_results_19.tex <==

\begin{tabular}{llllccccl}
\multicolumn{1}{c}{\multirow{3}{*}{Structure}} &
\multicolumn{1}{c}{\multirow{3}{*}{Models}} &\multicolumn{2}{c}{Modes} && \multicolumn{2}{c}{Accuracy} &&  \\     
\cline{3-4} \cline{6-7} 

\multicolumn{1}{c}{} & &  \multirow{2}{*}{HP} & \multirow{2}{*}{LP} && \multirow{2}{*}{HP} & \multirow{2}{*}{LP} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}KL\\ divergence\end{tabular}} & Time (sec)\\
\multicolumn{1}{c}{}   & &  &         \\ \hline

\multicolumn{1}{c}{\multirow{7}{*}{FF}} &
GAN \citep{goodfellow2014generative}& 13,148 $\pm$ 7,349 & 6,351 $\pm$ 3,135  &&  0.3374 $\pm$ 0.0911 & 0.6576 $\pm$ 0.0942 & 0.07343 $\pm$ 0.05317 & 439 $\pm$ 12\\
&GAN + MB \citep{salimans2016improved} & 9,698 $\pm$  5,824 &  4,443 $\pm$ 2,139 &&  0.3621 $\pm$ 0.1208 & 0.6260 $\pm$ 0.1191 & 0.06655 $\pm$ 0.03573 & 448 $\pm$ 29\\	
% DSGAN && 14,218 $\pm$ 7,110 & 4,085 $\pm$ 2,454 && 0.1783 $\pm$ 0.0519 & 0.8220 $\pm$ 0.0598 & 0.22780 $\pm$ 0.09041\\

&PacGAN \citep{lin2018pacgan} & 2,232 $\pm$ 1,271 & 1,078 $\pm$ 741 && 0.4046 $\pm$ 0.3167 & 0.5928 $\pm$ 0.3152 & 0.26998 $\pm$  0.25194 & 369 $\pm$ 30\\

&MAD-GAN \citep{ghosh2018multi} &- & - && - & - & -\\
&GDPP \citep{elfeki2019gdpp} & 5,232 $\pm$ 5,206 & 2,625 $\pm$ 1,196 && 0.4412 $\pm$ 0.2078 & 0.5669 $\pm$ 0.2069 & 0.09441 $\pm$ 0.07688 & 1,241 $\pm$ 38\\
\cline{2-9}


&VARGAN (Our approach) & 13,534 $\pm$ 6,718 & 5,204 $\pm$ 2,954 && 0.2784 $\pm$ 0.0917 & 0.7155 $\pm$ 0.0895 & 0.11176 $\pm$ 0.06120 & 673 $\pm$ 52\\
&PacVARGAN (Our approach + PacGAN) &  11,266 $\pm$ 3,077 & 4,476 $\pm$ 1,696 && 0.2810 $\pm$ 0.0426 &  0.7153 $\pm$ 0.0443 &  0.10882 $\pm$ 0.03999 & 637 $\pm$ 21	\\	
\midrule
\multicolumn{1}{c}{\multirow{7}{*}{Conv}} &
GAN \citep{goodfellow2014generative}&  237 $\pm$ 229 & 258 $\pm$ 346 && 0.6799 $\pm$ 0.2050 & 0.3216 $\pm$ 0.2050 & 0.17950 $\pm$ 0.22395 & 975 $\pm$ 60	\\

&GAN + MB \citep{salimans2016improved}& 521 $\pm$ 611 & 550 $\pm$ 670 && 0.6138 $\pm$ 0.2615 & 0.3839 $\pm$ 0.2600  &0.20468 $\pm$ 0.25432 & 3,766 $\pm$ 60\\

% DSGAN && 428 $\pm$ 365 & 776 $\pm$ 403 &&  0.8099 $\pm$ 0.1435 & 0.1883 $\pm$ 0.1409 &	0.28596 $\pm$ 0.23887\\
&PacGAN \citep{lin2018pacgan} & 15,343  $\pm$  1,180  & 7,260  $\pm$  1,714&& 0.6805  $\pm$ 0.0442 & 0.3193  $\pm$ 0.0471 &  0.07148 $\pm$  0.03324 & 908 $\pm$ 11\\
&MAD-GAN \citep{ghosh2018multi} & 3,166 $\pm$  2,037 &  689 $\pm$  860  && 0.0275 $\pm$  0.0477 & 0.1431 $\pm$  0.1108 & 0.26012 $\pm$  0.08118 & 2,256 $\pm$ 39\\
&GDPP \citep{elfeki2019gdpp} &  501 $\pm$ 451 & 271 $\pm$ 329 && 0.7499 $\pm$ 0.3189 & 0.2509 $\pm$ 0.3192 & 0.42096 $\pm$ 0.24309 & 1,562 $\pm$ 73 \\
\cline{2-9}
 &VARGAN (Our approach)& 1,848 $\pm$ 1,316  & 896 $\pm$ 415 && 0.6114  $\pm$  0.2360 & 0.3878 $\pm$ 0.2379 & 0.15896  $\pm$ 0.18456 & 578 $\pm$  50\\

% &VARGAN (Our approach)&   355 $\pm$ 430 & 152 $\pm$ 199  && 0.7301 $\pm$  0.2890& 0.2705 $\pm$  0.2900 &0.31770 $\pm$  0.15069 & 1,219 $\pm$ 45 \\
% &PacVARGAN (Our approach + PacGAN) &15,585  $\pm$   1,874 & 7,272 $\pm$ 1,094 && 0.6980 $\pm$ 0.0187 &0.3009 $\pm$ 0.0203 & 0.08195 $\pm$ 0.01710 & 1,126 $\pm$ 12\\
 &PacVARGAN (Our approach + PacGAN) & 13,965 $\pm$  1,039 & 5,318  $\pm$  1,606 && 0.7399  $\pm$ 0.0672 &
0.2574  $\pm$  0.0696 & 0.13430 $\pm$  0.08211 &  467 $\pm$  50\\
\bottomrule
\end{tabular}






==> Tables/Experimental_setup_EES.tex <==

% \begin{tabular}{|c|c|c|c|p{0.5cm}|c|c|c|c|p{0.5cm}|p{0.6cm}|p{0.6cm}|c|c|}
\noindent\adjustbox{max width=\textwidth}{

\begin{tabular}{ccrcccccccccc}
 \multirow{6}{*}{Structure} &  
 \multirow{6}{*}{Model} &
 \multicolumn{9}{c}{Category Names} &&  \multirow{6}{*}{KL}\\
 \cline{3-11}
 & & \multicolumn{5}{c}{HP} &  \multirow{4}{*}{SUM} &\multicolumn{3}{c}{LP}& \multirow{4}{*}{SUM}\\
 \cline{3-7}
 \cline{9-11}
 &  &  DC Block  & DC Block  & DC Block  & DC Block & DC Block&  & DC Pass  & DC Pass & DC Pass\\
 & &  Band Pass & Band Pass Stop & High Pass & True High Pass &  Very High Pass & &Band Stop & Low Pass & Stop Pass\\
\toprule
% \multirow{2}{*}{cGAN}&  \multirow{2}{*}{$9\times9$} & Total in data & 2,804 & 2,614 & 3,206 & 8,556 & 5,537 &22,717& 4,193 & 4,467 & 1,391 & 10,051\\
% & && 1,272 & 1,383 & 1,819 & 5,819 & 2,934 &13,227& 2,851 & 2,400 & 750& 6,001\\
% & & \% & 45 & 53 & 57 & 68 & 53 & 58 & 68 & 54 & 54 & 59\\
% \midrule
% \multirow{2}{*}{cGAN}&  \multirow{2}{*}{$9\times9$} & DSGAN  & 1,803 & 1,757 & 2,434 & 5,785 & 3,910 & 15,689 & 3,340 & 3,201 & 961 & 7,502 & 0.0729 $\pm$ 0.0031\\
% & & \% & 79 & 75 & 69 & 68 & 70 & 70 & 67 & 64 & 67 & 75\\
% \midrule
% \multirow{2}{*}{cGAN}&  \multirow{2}{*}{$9\times9$} & MB Discr & 1,106 & 1,241& 1,563& 4,802 & 2,224 & 10,936 & 2,444 & 2,088 & 609 & 5,141 &0.0936 $\pm$ 0.0047\\
% & & \% & 40 & 47 & 49 & 56 & 40 & 48 & 58 & 47 & 43 & 51\\
% \midrule
% \multirow{2}{*}{cGAN}&  \multirow{2}{*}{$9\times9$} & PacGAN  & 747& 805 & 974 & 2,609 & 1,629 & 6,764 & 1,579 & 1,435 &  427 & 3,441 & 0.0304 $\pm$ 0.0128\\
% & & \% & 27 & 31 & 30 & 30 & 30 & 30 & 38 & 32 & 31 & 34 \\
% \midrule
% \midrule
% \multirow{2}{*}{cCGAN}& 
% \multirow{2}{*}{$9\times9$} & Total in data & 2,804 & 2,614 & 3,206 & 8,556 & 5,537 &22,717& 4,193 & 4,467 & 1,391 & 10,051\\
% & & 8 Categories & 2,275 & 2,204& 2,653 & 7,061 & 4,574 &18,867& 3,538 & 3,765 & 1,175& 8,478 \\
% & & \% & 81 & 84 & 83 & 82 & 83 &83 & 84 & 84 & 84& 84 \\
% \midrule
% \multirow{2}{*}{cCGAN}&  \multirow{2}{*}{$9\times9$} & DSGAN  &2,664 & 2,531 & 3,035 & 8,322 & 5,344& 21,896 & 3,994 & 4,353 & 1,342 & 9,689 & 0.0033 $\pm$ 0.0018\\
% & & \% & 95 & 97 & 95 & 97 & 96 &96& 95 & 97 & 96 &96 \\
% \midrule
% \multirow{2}{*}{cCGAN}&  \multirow{2}{*}{$9\times9$} & MB Discr & 2,686 & 2,511 & 3,047 & 8,258 & 5,283 & 21,785 & 3,929 & 4,269 & 1,329 & 9,527 & 0.0020 $\pm$ 0.0014\\
% & & \% & 96 & 96 & 95 & 96 & 95 & 96 & 94 & 96 & 95 & 95\\
% \midrule
% \multirow{2}{*}{cCGAN}&  \multirow{2}{*}{$9\times9$} & PacGAN  & 2,740 & 2,566 & 3,130 & 8,359 & 5,399 & 22,194 & 4,026  & 4,370 & 1,366 & 9,762 & 0.0015 $\pm$ 0.0010\\
% & & \% & 98 & 98 & 98 & 98 & 97 & 98 & 96 & 98 & 98 & 97 \\
% \midrule
% \midrule
% \multirow{2}{*}{GAN}& 
% \multirow{2}{*}{$9\times9$} & Total in data & 2,804 & 2,614 & 3,206 & 8,556 & 5,537 &22,717& 4,193 & 4,467 & 1,391 & 10,051\\
% & & 8 Categories & 2,682 &  2,501 &  3,050 &  8,146 &  5,265 & 21,644 &  4,000 &  4,278&  1,340 &  9,618 & 0.0007 $\pm$ 0.0003\\
% & & \% & 96 & 96 & 95 & 95 & 95 & 95 & 95 & 96 & 96 & 96\\
% \midrule
% \multirow{2}{*}{GAN}& 
% \multirow{2}{*}{$9\times9$} & DSGAN &  2,613 & 2,422 & 2,999 &  8,019 &  5,148 & 21,201 &  3,907 &  4,165 & 1,297 & 9,369 & 0.0012 $\pm$ 0.0007 \\
% & & \% & 93 & 93 & 94 & 94 & 93 & 93 & 93 & 93 & 93 & 93\\
% \midrule
% \multirow{2}{*}{GAN}& 
% \multirow{2}{*}{$9\times9$} & MB Discr & 2,683 &  2,503 &  3,065 &  8,172 &  5,262 & 21,685 &  4,016 &  4,271 &  1,327 &  9,614 & 0.0008 $\pm$ 0.0007\\
% & & \% & 96 & 96 & 96 & 96 & 95 & 95 & 96 & 96 & 95& 96\\
% \midrule
% \multirow{2}{*}{GAN}& 
% \multirow{2}{*}{$9\times9$} & PacGAN &  997 &  918 &  1,139 &  2,981 &  1,939 &  7,974 &  1,507 &  1,504 &   474 &  3,485 & 0.0142 $\pm$ 0.0115 \\
% & & \% & 36 & 35 & 36 & 35&35 &35& 36& 34& 34& 35\\
% \midrule
% \midrule

\multirow{6}{*}{Conv}&
GAN& 2,521 $\pm$ 238 &
2,410 $\pm$ 116 &
2,945 $\pm$ 169 &
7,819 $\pm$ 446 &
5,093 $\pm$ 311 & 20,788&
3,788 $\pm$ 231 &
4,083 $\pm$ 266 &
1,278 $\pm$ 73 & 9,149 & 0.00407 $\pm$ 0.00283\\
% GAN& 2,700  $\pm$ 16 & 2,524 $\pm$ 18 & 3,099 $\pm$ 15& 8,265 $\pm$ 49& 5,353 $\pm$ 22& 21,941 & 4,055 $\pm$ 33& 4,321 $\pm$ 24& 1,348 $\pm$ 12 &9,724& 0.00134 $\pm$  0.00123\\
% & & \% & 96 & 97 & 97 & 97 & 97& 97& 97& 97& 97& 97\\
% && Accuracy & \\
% &  MSGAN & 2,720 $\pm$ 25 & 2,507 $\pm$ 27 &  3,097 $\pm$ 11 &  8,265 $\pm$ 62 &  5,336 $\pm$ 26 & 21,925 & 4,049 $\pm$ 21 & 4,319 $\pm$ 25 & 1,335 $\pm$ 20 & 9,703 & 0.00180 $\pm$ 0.00135\\
% && Accuracy & \\
% & & \% &97 & 96 & 97 & 97 & 96 & 97 & 97 & 97 & 96 & 97 \\
% &  MB Discr & 2,714 $\pm$ 15 & 2,508 $\pm$ 25 &  3,091 $\pm$ 15 &  8,226 $\pm$ 58 & 5,345 $\pm$ 29 & 21,884 &  4,007 $\pm$ 34 &  4,300 $\pm$ 22 &  1,346 $\pm$ 8 &  9,653 & 0.00169 $\pm$ 0.00050\\
% && Accuracy & \\
% & & \% & 97 & 96 & 96 & 96 & 97 & 96 & 96 & 96& 97& 96\\
& MSGAN & 2,664 $\pm$ 35 &
2,531 $\pm$ 20 &
3,035 $\pm$ 45 &
8,322 $\pm$ 27 &
5,344 $\pm$ 28 & 21,896& 
3,994 $\pm$ 45 &
4,353 $\pm$ 17 &
1,342 $\pm$ 5 & 9,689 & 0.00337 $\pm$ 0.00183\\
&  PacGAN & 2,740 $\pm$ 15 &
2,566 $\pm$ 12 &
3,130 $\pm$ 14 &
8,359 $\pm$ 25 &
5,399 $\pm$ 23 &
22,194 &
4,026 $\pm$ 32 &
4,370 $\pm$ 24 &
1,366 $\pm$ 6 & 9,762 & 0.00156 $\pm$  0.00100\\
\cline{2-13}
& VARGAN & 1,543 $\pm$ 1,170 &
1,452 $\pm$ 1,116 &
1,730 $\pm$ 1,323 &
4,706 $\pm$ 3,665 &
2,933 $\pm$ 2,350 & 12,364 &
2,216 $\pm$ 1,758 &
2,465 $\pm$ 1,959 &
761 $\pm$ 581 & 5,442 & 0.08914 $\pm$ 0.10644\\
& PacVARGAN & 2,605 $\pm$ 279 &
2,479 $\pm$ 166 &
2,972 $\pm$ 317 &
8,011 $\pm$ 613 &
5,101 $\pm$ 622 & 21,168 &
3,816 $\pm$ 373 &
4,090 $\pm$ 537 &
1,265 $\pm$ 182 & 9,171 & 0.00394 $\pm$ 0.00431\\
% &  PacGAN & 2,719 $\pm$ 23 &  2,528 $\pm$ 16 &  3,099$\pm$ 20 &  8,265 $\pm$ 54 &  5,345 $\pm$ 42 & 21,956 &  4,061 $\pm$ 25 &  4,315 $\pm$ 28 &  1,353 $\pm$ 5&  9,729 & 0.00058  $\pm$ 0.00016\\
% && Accuracy & \\
% & & \% & 97 &97 &97 &97 &97 & 97 & 97 &97 & 97 & 97\\
% \cline{2-13}
% &  VARGAN &\\
% % && Accuracy & \\
% % & & \% \\
% &  PacVARGAN &\\
% &  VARGAN &  2,721 $\pm$ 8 &
% 2,516$\pm$ 14&
% 3,094 $\pm$ 3 &
% 8,260 $\pm$ 42 &
% 5,344 $\pm$ 21  & 21,935 & 4,052 $\pm$ 23 &
% 4,312 $\pm$ 20 &
% 1,346 $\pm$ 9 & 9,710 & 0.00047 $\pm$ 0.00036\\
% % && Accuracy & \\
% % & & \% \\
% &  PacVARGAN & 2,697 $\pm$ 18 &
% 2,514 $\pm$ 20 &
% 3,079 $\pm$ 29 &
% 8,246 $\pm$ 54 &
% 5,319 $\pm$ 21 & 21,855 & 4,007 $\pm$ 53 & 4,277 $\pm$ 23 &
% 1,347 $\pm$ 10 & 9,631 & 0.00218 $\pm$ 0.00198

% && Accuracy & \\
% & & \% \\
\midrule
Total samples in & input data & 2,804 & 2,614 & 3,206 & 8,556 & 5,537 &22,717& 4,193 & 4,467 & 1,391 & 10,051\\

% etc. ...
\end{tabular}}

==> Tables/Experimental_setup_MNIST.tex <==
\begin{tabular}{lllllllllllll}
\toprule
                   & GAN architecture               & \multicolumn{2}{c}{MNIST} & & \multicolumn{2}{l}{Binary MNIST}  && \multicolumn{2}{c}{MNIST} & & \multicolumn{2}{l}{Binary MNIST} \\ 
                                  \cline{3-4} \cline{6-7} \cline{9-10} \cline{12-13}
                                  & &Modes (Max 10)     & KL &   & Mode (Max 10)         & KL    & &Modes (Max 2)     & KL &   & Mode (Max 2)         & KL      \\ \hline
\multicolumn{1}{l}{-} & cCGAN\\

\bottomrule
\end{tabular}


==> Tables/New_mode_collapse_Stacked_MNIST.tex <==
\begin{tabular}{lllllll}
\toprule
                   & GAN architecture               & \multicolumn{2}{c}{Stacked MNIST} & & \multicolumn{2}{l}{Stacked Binary MNIST} \\ 
                                  \cline{3-4} \cline{6-7} 
                                  & &Modes (Max 1000)     & KL &   & Mode (Max 10)         & KL        \\ \hline
\multicolumn{1}{l}{z =100} & cGAN &   600  &  0.640 $\pm$ 0.008   & & 202 & 2.102 $\pm$ 0.062   \\
\multicolumn{1}{l}{z =500} & cGAN& 604 & 0.636 $\pm$ 0.016& & 200&2.095 $\pm$ 0.036\\
\multicolumn{1}{l}{z =1000} & cGAN & 609 & 0.625 $\pm$ 0.018& &190 & 2.203 $\pm$ 0.031\\
\multicolumn{1}{l}{z =5000} & cGAN & 617 & 0.606 $\pm$ 0.011& & 202 & 2.084 $\pm$ 0.027\\

\multicolumn{1}{l}{z =100} & cCGAN&   \\
\multicolumn{1}{l}{z =500} & cCGAN&  \\
\multicolumn{1}{l}{z =1000} & cCGAN \\
\multicolumn{1}{l}{z =5000} & cCGAN\\
\midrule
\multicolumn{1}{l}{z =100, Reslayers} & cGAN& 627 & 0.583 $\pm$ 0.014\\\
\multicolumn{1}{l}{z =100, Reslayers} & cCGAN&\\

\bottomrule
\end{tabular}


==> Tables/New_mode_collapse_ideas.tex <==
\begin{tabular}{lllllll}
\toprule
                   & GAN architecture               & \multicolumn{2}{c}{MNIST} & & \multicolumn{2}{l}{Binary MNIST} \\ 
                                  \cline{3-4} \cline{6-7} 
                                  & &Modes (Max 10)     & KL &   & Mode (Max 10)         & KL        \\ \hline
\multicolumn{1}{l}{z =100} & cGAN&10& 0.076 $\pm$ 0.007 & &10& 0.127 $\pm$ 0.005    \\
\midrule
\multicolumn{1}{l}{z =500} & cGAN&10& 0.072 $\pm$ 0.029 & &10& 0.125 $\pm$ 0.044 \\
\multicolumn{1}{l}{z =1000} & cGAN&10& 0.063 $\pm$ 0.025 && 10&  0.098 $\pm$ 0.033\\
\multicolumn{1}{l}{z =5000} & cGAN&10& 0.060 $\pm$ 0.024&& 10& 0.130 $\pm$ 0.038\\
\midrule
\multicolumn{1}{l}{z =100} & cCGAN&  10& 0.005 $\pm$ 0.002& &10 &  0.133 $\pm$ 0.079  \\
\midrule
\multicolumn{1}{l}{z =500} & cCGAN&  \\
\multicolumn{1}{l}{z =1000} & cCGAN \\
\multicolumn{1}{l}{z =5000} & cCGAN\\
\midrule
\multicolumn{1}{l}{z =100, Reslayers} & cGAN&10& 0.025 $\pm$ 0.012\\
\multicolumn{1}{l}{z =100, Reslayers} & cCGAN&\\
% \multicolumn{1}{l}{z =500, Reslayers} & cGAN&10& 0.024 $\pm$ 0.012 \\
% \multicolumn{1}{l}{z =1000, Reslayers} & cGAN&10& 0.026 $\pm$ 0.012\\
% \multicolumn{1}{l}{z =5000, Reslayers} & cGAN&10& 0.025 $\pm$ 0.011\\
\bottomrule
\end{tabular}


==> Tables/Result_VAR_compare_grid.tex <==


\begin{tabular}{m{0.09\textwidth}m{0.11\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}}
% \rowcolor[HTML]{FFF} 
% {\textbf{stat}} & { \textbf{Model-name}} & {\color[HTML]{212121} \textbf{Modes thresh}} & {\color[HTML]{212121} \textbf{Modes nonthresh }} & {\color[HTML]{212121} \textbf{KL thresh}} & {\color[HTML]{212121} \textbf{KL score}} & {\color[HTML]{212121} \textbf{KL nonthresh}} & {\color[HTML]{212121} \textbf{KL nonthresh score}} & {\color[HTML]{212121} \textbf{High quality samples }} \\
\toprule
{Epoch} & { Model} & { Modes with thresh} & {  Modes without thresh}& { KL thresh} &{ KL score} & { KL nonthresh} & { KL nonthresh score} & { High quality samples }\\[1.5em]
\midrule
 400      & GAN      & 25.0  & 25.0 & 0.4588 & 0.1180  & 0.3704 & 0.0952 & 0.8526 \\
% 1   & GAN      & 5.0   & 8.8  & 2.3164 & 0.2202 & 1.7288 & 0.1828 & 0.4098 \\
50  & GAN      & 24.8  & 25.0 & 0.1796 & 0.0454 & 0.1316 & 0.0346 & 0.7140  \\
% 104 & GAN      & 25.0  & 25.0 & 0.2876 & 0.073  & 0.2174 & 0.0552 & 0.806  \\
% 155 & GAN      & 25.0  & 25.0 & 0.3296 & 0.0824 & 0.25   & 0.0624 & 0.812  \\
 400     & VARNET   & 25.0  & 25.0 & 0.3376 & 0.0902 & 0.2784 & 0.0736 & 0.8636 \\
% 1   & VARNET   & 20.6  & 21.8 & 0.79   & 0.131  & 0.5794 & 0.1072 & 0.4134 \\
50  & VARNET   & 25.0  & 25.0 & 0.1040  & 0.0276 & 0.0824 & 0.0216 & 0.8220  \\
% 104 & VARNET   & 25.0  & 25.0 & 0.2092 & 0.0562 & 0.1634 & 0.043  & 0.854  \\
% 155 & VARNET   & 25.0  & 25.0 & 0.2434 & 0.0664 & 0.2102 & 0.0568 & 0.896  \\
400      & PacGAN      & 25.0  & 25.0 & 0.1560  & 0.0402 & 0.1150  & 0.0290  & 0.6632 \\
% 1   & pac      & 10.2  & 13.2 & 1.9476 & 0.224  & 1.5516 & 0.2048 & 0.448  \\
50  & PacGAN      & 24.4  & 24.8 & 0.2184 & 0.0500   & 0.1346 & 0.0334 & 0.6040  \\
% 104 & pac      & 24.6  & 24.8 & 0.1908 & 0.0452 & 0.1368 & 0.0346 & 0.608  \\
% 155 & pac      & 24.8  & 25.0 & 0.1468 & 0.0356 & 0.0966 & 0.025  & 0.604  \\
400      & Pac-VAR & 25.0  & 25.0 & 0.1070  & 0.0275 & 0.0668 & 0.0170  & 0.7475 \\
% 1   & pacvar & 10.25 & 13.5 & 1.6405 & 0.1945 & 1.235  & 0.16   & 0.4765 \\
50  & Pac-VAR & 25.0  & 25.0 & 0.1130  & 0.0292 & 0.0628 & 0.0158 & 0.6225 \\
% 104 & pacvar & 25.0  & 25.0 & 0.113  & 0.0295 & 0.078  & 0.0205 & 0.625  \\
% 155 & pacvar & 25.0  & 25.0 & 0.14   & 0.0358 & 0.0782 & 0.02   & 0.6075\\
\end{tabular}


==> Tables/Result_VAR_compare_ring.tex <==


\begin{tabular}{m{0.09\textwidth}m{0.11\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}m{0.09\textwidth}}
% \rowcolor[HTML]{FFF} 
% {\textbf{stat}} & { \textbf{Model-name}} & {\color[HTML]{212121} \textbf{Modes thresh}} & {\color[HTML]{212121} \textbf{Modes nonthresh }} & {\color[HTML]{212121} \textbf{KL thresh}} & {\color[HTML]{212121} \textbf{KL score}} & {\color[HTML]{212121} \textbf{KL nonthresh}} & {\color[HTML]{212121} \textbf{KL nonthresh score}} & {\color[HTML]{212121} \textbf{High quality samples }} \\
\toprule
{Epoch} & { Model} & { Modes with thresh} & {  Modes without thresh}& { KL thresh} &{ KL score} & { KL nonthresh} & { KL nonthresh score} & { High quality samples }\\[1.5em]
\midrule
400 & GAN & 6.2     & 8.0       & 0.6906       & 0.1272      & 0.5958  & 0.1708  & 0.8758       \\
 50& GAN     & 4.6     & 7.2       & 0.7736       & 0.0772      & 0.5590   & 0.1274  & 0.4620\\
400   & VARNET  & 7.0     & 8.0       & 0.6532       & 0.1594      & 0.5360   & 0.1588  & 0.8772       \\

 53& VARNET  & 4.4     & 8.0       & 0.7322       & 0.0658      & 0.5104  & 0.1462  & 0.6880\\

400   & PacGAN     & 8.0     & 8.0       & 0.0368       & 0.0096      & 0.0074  & 0.0020   & 0.7116       \\

 50& PacGAN     & 7.6     & 8.0       & 0.3398       & 0.0764      & 0.0062  & 0.0012  & 0.2500 \\

400   & Pac-VAR & 8.0     & 8.0       & 0.1604       & 0.0438      & 0.0080   & 0.0020   & 0.5276       \\

 50& Pac-VAR & 7.4     & 8.0       & 0.3158       & 0.0604      & 0.0056  & 0.0014  & 0.2160\\

\end{tabular}


==> Tables/Results-Stacked-MNIST.tex <==
\begin{tabular}{lllllll}
\toprule
                 &GAN architecture                & \multicolumn{2}{c}{Stacked MNIST} & & \multicolumn{2}{l}{Binary Stacked MNIST} \\ 
                                  \cline{3-4} \cline{6-7} 
                                  & &Modes (Max 1000)     & KL &   & Mode (Max 1000)         & KL        \\ \hline
- &\multicolumn{1}{l}{cCGAN} &   55   & 4.074$\pm$ 0.019 && 342&  1.230$\pm$ 0.091     \\
- &\multicolumn{1}{l}{CGAN}&   406   & 1.216$\pm$ 0.076 && 569 &0.717$\pm$0.013     \\
- &\multicolumn{1}{l}{cGAN} &   600  &  0.640 $\pm$ 0.008   & & 202 & 2.102 $\pm$ 0.062   \\
% \multicolumn{1}{l}{GAN}   &     &  302 & 1.716 $\pm$ 0.037 && 451 &   1.043 $\pm$ 0.029   \\
- &\multicolumn{1}{l}{GAN} &  518  & 0.849 $\pm$ 0.040 &  &  210& 1.998   $\pm$  0.076 \\
\midrule
\multicolumn{1}{l}{PacGAN} & cGAN\\
\multicolumn{1}{l}{DSGAN} & cGAN & 627 & 0.583 $\pm$  0.020 && 203 & 2.075 $\pm$  0.065\\
\midrule
% \multicolumn{1}{l}{Unrolled GAN} &  -    &  - &&   - & -    \\
\multicolumn{1}{l}{DSGAN} & cCGAN &\\
\multicolumn{1}{l}{MB Discr} &   cCGAN    &   393   &  1.008 $\pm$0.006 &&393&1.008$\pm$0.007 \\
\multicolumn{1}{l}{VEEGAN} &cCGAN      &   -   &  - &&  -  & -  \\

\multicolumn{1}{l}{PacGAN} &cCGAN&  53    &   4.141$\pm$0.0949&& 132   & 2.563$\pm$0.087  \\

\midrule
% \multicolumn{1}{l}{Unrolled GAN} &  -    &  - &&   - & -    \\
\multicolumn{1}{l}{MB Discr} &   CGAN   &415&1.145$\pm$0.097&&585&0.679$\pm$0.011 \\
\multicolumn{1}{l}{VEEGAN} &CGAN      &   -   &  - &&  -  & -  \\

\multicolumn{1}{l}{PacGAN} &CGAN&  434    &   1.114$\pm$0.067&& 555   &  0.749$\pm$0.054 \\

\multicolumn{1}{l}{Our GAN} &    -  &  - &&  -  &      -    \\
\bottomrule
\end{tabular}


==> Tables/VARNET-StackedMNIST.tex <==
\noindent\adjustbox{max width=\textwidth}{

\begin{tabular}{c|c|ccc}
\toprule
 \multirow{3}{*}{Epoch} &\multirow{3}{*}{Model} &  \multicolumn{3}{c}{Stacked MNIST} \\
 \cline{3-5}
 &  & Modes & reverse KL & Inception Score\\
 & & (Max 1000) & &\\
\toprule
4 & GAN &619& 1.23 &1.97\\
5 & GAN &482 & 1.73 & 1.62\\
6 & GAN & 440& 2.20 & 1.63\\
4& PacGAN & 626 & 1.08 & 2.02\\
5& PacGAN & 640 & 1.04 & 1.95\\
6& PacGAN & 659 & 0.95 & 1.99\\
\midrule
4& VAR-GAN & 792 & 0.44 & 2.27\\
5& VAR-GAN & 683 & 1.056 & 2.04\\
6& VAR-GAN & 618 & 1.06 & 1.88\\

4& VAR-PacGAN & 604 & 1.13 & 1.88\\
5& VAR-PacGAN & 617 & 0.93 & 1.77\\
6& VAR-PacGAN & 545 & 1.35 &1.71\\

\end{tabular}}

==> Tables/VAR_synthetic_data.tex <==
\noindent\adjustbox{max width=\textwidth}{

\begin{tabular}{c|c|cccccccccccccccccccccc}
\toprule
\multirow{3}{*}{Epoch} & \multirow{3}{*}{Model} & 
 \multicolumn{5}{c}{2D ring} && \multicolumn{5}{c}{2D grid} && \multicolumn{5}{c}{2D grid} \\
 \cline{3-7}
 \cline{9-13}
 \cline{15-19}
 & & Modes && High quality  && reverse  && Modes && High quality && reverse  && Modes && High quality && reverse  
\\
& & (Max 8) &&  samples && KL && (Max 25)&& samples && KL&& (Max 36)&& samples && KL\\
\toprule
50 & GAN & 4.6  && 46.20 && 0.77  && 24.8 &&71.40 &&0.17 && 33.8 && 70.00 &&0.34 \\
400 & GAN & 6.2 && 87.58  && 0.69 && 25.0&&85.26&&0.45 && 36.0 && 84.10 && 0.18\\

50 &PacGAN & 7.6 && 25.00 && 0.33 && 24.4 && 60.40 &&0.21 && 36.0 && 65.20 && 0.16\\
400 & PacGAN &  8.0 && 71.16 && 0.03 && 25.0&&66.32&&0.15&&36.0 &&72.40 && 0.09 \\

\midrule
50 &VARGAN & 4.4  && 68.80  && 0.73 &&  25.0&& 82.20 && 0.10 && 36.0 && 68.4 && 0.11 \\\
400 &VARGAN & 7.0 &&  87.72  && 0.65 &&  25.0&& 86.36 &&  0.33 && 36.0 && 88.22 && 0.20\\


50 &VARPacGAN &7.4  &&  21.60  && 0.31 && 25.0 && 62.25&& 0.11 && 36.0 && 67.40 && 0.14\\
400 & VARPacGAN &8.0  && 52.76   && 0.16 && 25.0 &&74.75 && 0.10 && 36.0 && 75.94 && 0.07\\

\end{tabular}}

 




==> Tables/comparison_EES.tex <==
\noindent\adjustbox{max width=\textwidth}{
\begin{tabular}{llcrrlll}
\toprule
                    GAN architecture              & Design & Category & \multicolumn{3}{c}{Partial Image}\\ 
                    % & & \multicolumn{3}{l}{Full Image} \\ 
                                  \cline{4-6}  
                                   & & &HP     & LP & KL \\ \hline
                                  

% - &GAN& $9\times9$ & & 4,230 &3,025 & &2,650 & 1,417\\
\midrule
cGAN& $9\times9$ & - &11,402 &6,251 & 0.0725 $\pm$ 0.0019 & &     \\
% 0.0002 $\pm$ 0.0000
% 

cGAN& $9\times9$ & DSGAN&  11,659 & 6,708 & 0.0707 $\pm$  0.0025\\
% 0.0003 $\pm$ 0.0001
cGAN& $9\times9$ &  MB Discr&  11,460 & 6,430 &  0.0532 $\pm$ 0.0298 \\
% 0.0117 $\pm$ 0.0228
cGAN& $9\times9$ &  PacGAN& 5,595 & 2,984 & 0.0255 $\pm$ 0.0085 \\
% 0.0160 $\pm$ 0.0059
cGAN& $9\times9$ & VARNET, coef = 0.7 & 11,469 & 6,315 & 
0.0723 $\pm$ 0.0021\\
\midrule

cCGAN& $9\times9$ & - & 10,909 & 5,147 &    0.0061 $\pm$ 0.0067\\
cCGAN& $9\times9$ & DSGAN & 14,612 & 7,452 & 0.0151 $\pm$ 0.0023\\
% 0.0252 $\pm$ 0.0032 
cCGAN& $9\times9$ & MB Discr &  14,814 & 7,089 & 0.0041 $\pm$ 0.0016\\ 
% 0.0468 $\pm$ 0.0053
cCGAN& $9\times9$ & PacGAN & 10,549 & 4,912 & 0.0074 $\pm$ 0.0047 \\
cCGAN& $9\times9$ & VARNET, coef = 1 & 15,163 & 7,205 & 0.0031 $\pm$ 0.0016\\
% 0.0397 $\pm$ 0.0098
\midrule
GAN& $9\times9$ & - & 14,518 & 6,369 & 0.0003 $\pm$ 0.0004 \\
GAN& $9\times9$ & DSGAN& 14,321 & 6,121 & 0.0018 $\pm$ 0.0019\\ 
GAN& $9\times9$ & MB Discr& 16,882 & 6,464 & 0.0001 $\pm$ 0.0001 \\
GAN& $9\times9$ &  PacGAN& 2,368 & 958 & 0.0034 $\pm$ 0.0041 \\
GAN& $9\times9$ & VARNET, coef = 0.8
 &14,884 &  6,498 & 0.0003 $\pm$ 0.0002\\
\midrule
CGAN& $9\times9$ & - & 14,843 & 6,646 & 0.0005 $\pm$ 0.0004 \\
CGAN& $9\times9$ & DSGAN & 14,897 & 6,511 & 0.0006 $\pm$ 0.0005\\
CGAN& $9\times9$ & MB Discr  & 14,898 & 6,597 & 0.0002 $\pm$ 0.0001 \\
CGAN& $9\times9$ &  PacGAN& 14,995 & 6,610 & 0.0005 $\pm$ 0.0005\\
CGAN& $9\times9$ & VARNET, coef = 1 & 14,826 & 6,618 & 0.0009 $\pm$ 0.0001 \\
\midrule
- & $9\times9$ & Total in data & 22,717 & 10,051 \\
\midrule
\midrule

cGAN& $19\times19$ & - &4,126 & 9,673  & 0.2098 $\pm$ 0.2440\\
% 0 & 1,250 
cGAN& $19\times19$  & DSGAN &  4,366 & 8,882 & 0.3413 $\pm$ 0.2881\\
cGAN& $19\times19$ &  MB Discr & 3,526 & 11,257 & 0.1915 $\pm$ 0.2564\\
cGAN& $19\times19$  & PacGAN & 1,735 & 3,548 & 0.2149 $\pm$ 0.2453 & &\\
cGAN& $19\times19$ & VARNET, coef = 1 & 11,407 & 22,246 & 0.0544 $\pm$ 0.0355\\
\midrule
cCGAN& $19\times19$  & - & 595 & 400 & 0.3033 $\pm$ 0.3215& &\\
% 81 & 76
% 0.3033 0.3215605137450804
% [595. 400.]

cCGAN& $19\times19$  & DSGAN & 524 &535 & 0.2881 $\pm$ 0.3078 & &\\
cCGAN& $19\times19$  & MB Discr & 15,495 & 10,445& 0.2215 $\pm$ 0.2178\\
cCGAN& $19\times19$  & PacGAN & 18,127&6,382 & 0.1082 $\pm$ 0.0489&\\
cCGAN& $19\times19$ & VARNET, coef = 0.8 & 547& 478 & 0.1253 $\pm$ 0.1285\\
\midrule
GAN& $19\times19$ & - & 6,226 &  2,045 & 0.2196 $\pm$ 0.2503\\
GAN& $19\times19$ & DSGAN& 15,311 & 7,997 & 0.0506 $\pm$ 0.0239 \\
GAN& $19\times19$ & MB Discr & 7,920 & 4,144 & 0.0958 $\pm$ 0.0681 \\
GAN& $19\times19$ & PacGAN & 8,852 & 2,764 & 0.1419 $\pm$ 0.0973\\
GAN& $19\times19$ & VARNET, coef = 1 & 8,185 & 20,086& 0.1053 $\pm$ 0.0793\\
\midrule
CGAN& $19\times19$ & - & 112 &71 & 0.3422 $\pm$ 0.2922\\
CGAN& $19\times19$ & DSGAN& 350 & 163 & 0.3052 $\pm$ 0.2406\\
CGAN& $19\times19$ & MB Discr & 308 & 164 & 0.5510 $\pm$ 0.1637 \\
CGAN& $19\times19$ & PacGAN & 14,748 & 7,481 & 0.0699 $\pm$ 0.0430\\
CGAN& $19\times19$ & VARNET, coef = 0.8 & 708 & 391 & 0.1971 $\pm$ 0.1862\\
\midrule
- & $19\times19$ & Total in data  \\
\midrule
\midrule
cGAN& $39\times39$ & & \\
\midrule
cCGAN& $39\times39$ & &3315 &   3040 \\


\midrule
- &- & $39\times39$ & Total in data  \\
% \midrule
% \multicolumn{1}{l}{MB Discr}     & cCGAN &   10 & 0.004$\pm$0.000  &    & 10 &0.008$\pm$0.004 \\

% \multicolumn{1}{l}{VEEGAN}   & cCGAN     &  -      &-&    & - &- \\
% \multicolumn{1}{l}{PacGAN}  & cCGAN&   10 & 0.004$\pm$0.001& & 10   & 0.065$\pm$0.066    \\
% \midrule
% \multicolumn{1}{l}{MB Discr}     & CGAN &   10 & 0.043$\pm$0.005  &    & 10 & 0.111$\pm$0.047\\

% \multicolumn{1}{l}{VEEGAN}   & CGAN     &  -      &-&    &  -&- \\
% \multicolumn{1}{l}{PacGAN}  & CGAN&   10 & 0.030$\pm$0.006& & 10   & 0.089$\pm$0.004    \\
% \multicolumn{1}{l}{Our GAN} &      &   &    &      &\\
\bottomrule
\end{tabular}}

